StepGame: A New Benchmark for Robust Multi-Hop Spatial Reasoning in Texts

Inferring spatial relations in natural language is a crucial ability an intelligent system should possess. The bAbI dataset tries to capture tasks relevant to this domain (task 17 and 19). However, these tasks have several limitations. Most importantly, they are limited to fixed expressions, they are limited in the number of reasoning steps required to solve them, and they fail to test the robustness of models to input that contains irrelevant or redundant information. In this paper, we present a new Question-Answering dataset called StepGame for robust multi-hop spatial reasoning in texts. Our experiments demonstrate that state-of-the-art models on the bAbI dataset struggle on the StepGame dataset. Moreover, we propose a Tensor-Product based Memory-Augmented Neural Network (TP-MANN) specialized for spatial reasoning tasks. Experimental results on both datasets show that our model outperforms all the baselines with superior generalization and robustness performance.

==> tbls/statistics.tex <==
\begin{table}[!th]
\centering
\small
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l|lllll}
\hline
\hline
Noise Type & $k$=1 & $k$=2 & $k$=3 & $k$=4 & $k$=5 \\ \hline 
Supporting & 0.0 & 0.0 & 0.0 & 1.4 & 1.6 \\
Disconnected & 2.0 & 2.0 & 2.0 & 2.0 & 2.5 \\
Irrelevant & 1.0 & 1.5 & 1.5 & 1.5 & 2.0 \\ \hline
Total & 3.0 & 3.5 & 3.5 & 4.9 & 6.1 \\ \hline \hline
Noise Type & $k$=6 & $k$=7 & $k$=8 & $k$=9 & $k$=10 \\ \hline
Supporting & 1.7 & 1.9 & 2.0 & 2.1 & 2.1 \\
Disconnected & 2.5 & 2.5 & 3.0 & 3.0 & 3.0 \\
Irrelevant & 2.0 & 2.0 & 2.5 & 2.5 & 2.5 \\ \hline
Total & 6.3 & 6.4 & 7.5 & 7.6 & 7.6 \\ \hline \hline
\end{tabular}
\end{adjustbox}
\label{statistics}
\caption{The average number of nodes used for each type of distracting noise.}
\end{table}



==> tbls/step_game.tex <==
\begin{table*}[!t]
% \footnotesize
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lrrrrrr}
\hline
\hline
%\multicolumn{7}{c}{Test Accuracy for StepGame}                                                                                     %                                                    \\ \hline
Models & 
\multicolumn{1}{c}{$k=1$} & 
\multicolumn{1}{c}{$k=2$} & 
\multicolumn{1}{c}{$k=3$} & 
\multicolumn{1}{c}{$k=4$} & 
\multicolumn{1}{c}{$k=5$} & 
\multicolumn{1}{c}{Mean}           \\ \hline
RN~\cite{santoro2017simple}       & 44.43$\pm$4.00          & 33.20$\pm$3.65           & 23.74$\pm$2.35           & 17.90$\pm$1.15          & 14.80$\pm$2.41         & 26.81          \\
RRN~\cite{palm2018recurrent}      & 45.98$\pm$5.18          & 35.94$\pm$2.48           & 26.90$\pm$1.91           & 18.52$\pm$1.50          & 15.54$\pm$1.50         & 28.58          \\
UT~\cite{dehghani2018universal}   & 65.21$\pm$3.23          & 38.22$\pm$2.20           & 26.56$\pm$2.37           & 22.50$\pm$2.62          & 16.58$\pm$2.63         & 33.81          \\
STM~\cite{le2020self}             & 60.09$\pm$4.34          & 47.02$\pm$2.41           & 35.25$\pm$2.50           & 24.43$\pm$2.10          & 21.44$\pm$3.02         & 37.65          \\
TPR-RNN~\cite{schlag2018learning} & 90.08$\pm$2.38          & 58.26$\pm$3.77           & 45.72$\pm$3.83           & 34.70$\pm$4.48          & 29.30$\pm$3.07         & 51.61          \\\hline
TP-MANN                          & \textbf{96.98$\pm$0.20}  & \textbf{72.30$\pm$1.35} & \textbf{57.68$\pm$1.18} & \textbf{48.56$\pm$1.83} & \textbf{42.28$\pm$1.98} & \textbf{63.56} \\
\hline
\hline
\end{tabular}
\end{adjustbox}
\caption{Test accuracy on StepGame: Mean$\pm$Std over 5 runs. $k$ represents the size of the story.}% For each model, we use random seeds to run 10 times and average the best 5 results.}
\label{tbl:step_game}
\end{table*}

